Faster connectivity in low-rank hypergraphs via expander decomposition

We design an algorithm for computing connectivity in hypergraphs which runs in time $\hat O_r(p + \min\{\lambda^{\frac{r-3}{r-1}} n^2, n^r/\lambda^{r/(r-1)}\})$ (the $\hat O_r(\cdot)$ hides the terms subpolynomial in the main parameter and terms that depend only on $r$) where $p$ is the size, $n$ is the number of vertices, and $r$ is the rank of the hypergraph. Our algorithm is faster than existing algorithms when the the rank is constant and the connectivity $\lambda$ is $\omega(1)$. At the heart of our algorithm is a structural result regarding min-cuts in simple hypergraphs. We show a trade-off between the number of hyperedges taking part in all min-cuts and the size of the smaller side of the min-cut. This structural result can be viewed as a generalization of a well-known structural theorem for simple graphs [Kawarabayashi-Thorup, JACM 19]. We extend the framework of expander decomposition to simple hypergraphs in order to prove this structural result. We also make the proof of the structural result constructive to obtain our faster hypergraph connectivity algorithm.

==> min-cut-algo-backup.tex <==
\section{Algorithm}\label{sec:min-cut-algo}


In this section, we prove Theorem \ref{theorem:algo}. In Section \ref{sec:small-size-min-cut}, we give an algorithm to find a min-cut in hypergraphs where some min-cut has small size. In Section \ref{sec:large-min-cut}, we give an algorithm which uses the expander decomposition and the $\trim$ and $\shave$ operations defined in Section \ref{sec:trim-and-shave}  to find a min-cut if the size of every min-cut is large. In Section \ref{sec:main-algorithm}, we apply the sparsification algorithm of Chekuri and Xu, followed by a combination of our two algorithms in order to prove Theorem \ref{theorem:algo}.

\subsection{Small-sized Hypergraph Min-Cut}\label{sec:small-size-min-cut}
We recall that the size of a cut is the number of vertices on the smaller side of the cut. In this section, we give a randomized algorithm to find connectivity in hypergraphs in which some min-cut has size at most $s$. 
%for sufficiently small $s$. 
The following is the main result of this section. 

\begin{theorem}\label{thm:new-small-mincut-algo}
Let $s$ be a positive integer and let $G=(V,E)$ be an $r$-rank hypergraph of size $p$ that has a min-cut $(C,V \setminus C)$ with $|C| \leq s$. Then, there exists a randomized algorithm $\textsc{SmallSizeMinCut}$ which takes $G$ and $s$ as input and runs in time $\tilde{O}_r(s^{6r}p)$ to return a min-cut of $G$ with high probability.
%\knote{to return a min-cut of $G$ with high probability.} \cnote{It's not phrased this way because we want to say that the algorithm always returns a cut within the given runtime, and the ``whp" applies only to the cut being a min-cut. Maybe this isn't too important to emphasize, though?}
\end{theorem}

\begin{remark}
We note that the above result gives a randomized algorithm. In contrast, we give a simple but slightly slower deterministic algorithm for this problem in Appendix \ref{sec:det-small-size-min-cut}. 
\end{remark}

We prove Theorem \ref{thm:new-small-mincut-algo} using one of two possible algorithms based on the connectivity $\lambda$ of the input hypergraph: By Theorem \ref{thm:CX-approximation}, we can find a $k$ such that $\lambda \leq k \leq 3\lambda$ in $O(p)$ time. If $k \leq 2700s^r\log n$, then we use the algorithm from Theorem \ref{thm:small-lambda-small-cut} to find a min-cut in time $\tilde{O}_r(s^{3r}p + s^{6r})$ and if $k > 2700s^r \log n$ (i.e., $\lambda > 900s^r \log n$), then we use the algorithm from Theorem \ref{thm:big-lambda-small-cut} to find a min-cut in time $\tilde{O}_r(s^{3r}p)$.
These two algorithms exploit two slightly different ways of representing the hypergraph as a graph.

\subsubsection{Algorithm for small $\lambda$}
This section is devoted to proving the following theorem, which allows us to find a min-cut in a hypergraph with a small-sized min-cut. The algorithm is fast if the min-cut value is sufficiently small.

\begin{theorem}\label{thm:small-lambda-small-cut}
Let $s$ be a positive integer and let $G=(V,E)$ be an $r$-rank hypergraph of size $p$ that has a min-cut $(C,V \setminus C)$ with $|C| \leq s$. Then, there exists a randomized algorithm which takes $G$ and $s$ as input and runs in time $\tilde{O}_r(p\lambda^2rs^r + \lambda^4r^2s^{2r})$ to return a min-cut of $G$ with high probability.
\end{theorem}

In the rest of this subsection, let $s$ be a positive integer and let $G=(V, E)$ be an $r$-rank $n$-vertex hypergraph of with $m$ hyperedges and size $p$ that has a min-cut $(C, V\setminus C)$ with $|C|\le s$. Let $\lambda$ be the min-cut value of $G$ and let $k$ be the approximation of $\lambda$ obtained by running the algorithm from Theorem \ref{thm:CX-approximation}. If $p \leq 512k^2rs^r$, then $n \leq p \leq 512k^2rs^r$. In this case, we run the algorithm \textsc{SlowMinCut} from Theorem \ref{thm:slow-min-cut} to compute the min-cut in $G$ in time $O(np) = \tilde{O}(\lambda^4r^2s^{2r})$. Henceforth, we assume that $p > 512k^2rs^r$.%\danupon{Just curious. Where do we need this?} \cnote{We need this to guarantee that the BFS can't explore the whole graph without marking $512k^2rs^r$ edges.}


We construct an arc-weighted directed graph $D_G = (V_D, E_D)$ as follows: 
The vertex and arc sets of $D_G$ are given by $V_D := U_V \cup U_{E_{in}} \cup U_{E_{out}}$ and $E_D := E_1 \cup E_2$ respectively, where $U_V, U_{E_{in}}, U_{E_{out}}, E_1,$ and $E_2$ are defined next. 
The vertex set $U_V$ has a vertex $u_v$ for each $v \in V$. The vertex set $U_{E_{in}}$ has a vertex $e_{in}$ for every hyperedge $e \in E$, and the vertex set $U_{E_{out}}$ has a vertex $e_{out}$ for every hyperedge $e \in E$. The arc set $E_1$ has an arc $(e_{in}, e_{out})$ for every $e \in E$. The arc set $E_2$ has arcs $(v, e_{in})$ and $(e_{out}, v)$ for every $e \in E$ and $v \in e$. We assign a weight of $1$ to each arc in $E_1$ and a weight of $\infty$ to each arc in $E_2$. We note that $|V_D| = n + 2m$, and $|E_D| = m + 2p$. Furthermore, $D_G$ can be constructed from $G$ in $\tilde{O}(p)$ time.

\begin{definition}
A directed cut in $D_G$ is an ordered partition of the vertices into two parts $(C, V_D \setminus C)$ such that $\emptyset \neq C \cap U_V \neq U_V$, and its weight is the total weight of arcs outgoing from $C$.
\end{definition}

The following proposition relates min-cut in $G$ to min-weight directed cut in $D_G$.

\begin{proposition}\label{prop:reduction-to-directed-graph}
An algorithm that runs in time $\tilde{O}(f(p,s,r,\lambda))$ to find a min-weight directed cut in $D_G$, for some function $f$, can be used to find a min-cut in $G$ in time $\tilde{O}(p + f(p,s,r,\lambda))$.
\end{proposition}
\begin{proof}
We first note that every cut $(C, V \setminus C)$ in $G$ has a corresponding cut in $D_G$, namely $(C', V_D \setminus C')$ where $C' := \{u_v \colon v \in C\} \cup \{e_{in} \colon e \cap C \neq \emptyset \} \cup \{e_{out} \colon e \subseteq C\}$. The arcs cut by $(C', V_D \setminus C')$ will be arcs of the form $(e_{in}, e_{out})$ where $e \cap C \neq \emptyset$, but $e$ is not contained in $C$, and the number of such arcs is exactly the number of hyperedges in $\delta(C)$. Therefore, the min-weight of a directed cut in $D_G$ is at most the min-cut value in $G$.

Next, let $(C', V_D \setminus C')$ be a min-weight directed cut in $D_G$. Let $C := \{v \colon u_v \in C'\}$. We will show that $C' \cap U_{E_{in}} = \{e_{in} \colon e \cap C \neq \emptyset\}$ and $C' \cap U_{E_{out}} = \{e_{out} \colon e \subseteq C \}$. We note that a min-cut in $D_G$ must not cut any infinite cost hyperedges. Therefore, $C'$ must contain every vertex $e_{in}$ such that $e \cap C \neq \emptyset$. Similarly, $C'$ can contain a vertex $e_{out}$ only if $e \subseteq C$. Thus, $(C', V_D \setminus C')$ must cut all arcs $(e_{in}, e_{out})$ where $e \in \delta(C)$. Therefore, the min-weight of a directed cut in $D_G$ is at least the min-cut value in $G$. 

The above arguments imply that the min-weight of a directed cut in $D_G$ is equal to the min-cut value in $G$ and moreover, given a min-weight directed cut in $D_G$, we can recover a min-cut in $G$ immediately. The run-time guarantees follow. 
%The above arguments also allow us to recover a min

%and we conclude that the two graphs have the same min-cut value and their min-cuts are in correspondence.
\end{proof}

By Proposition \ref{prop:reduction-to-directed-graph}, in order to prove Theorem \ref{thm:small-lambda-small-cut}, it suffices to design an algorithm that runs in time $\tilde{O}_r(p\lambda^2rs^r + \lambda^4r^2s^{2r})$ to find a min-weight directed cut $(C, V_D \setminus C)$ in the directed graph $D_G$ corresponding to $G$, under the assumptions that $|C \cap U_V| \leq s$ and $p\ge 512k^2rs^r$. In Algorithm \ref{alg:s-sized-small-lambda} we give a randomized algorithm to find a min-weight directed cut under these assumptions.
%The rest of the section is devoted towards designing such an algorithm. 
Algorithm \ref{alg:s-sized-small-lambda} is inspired by an algorithm of Forster et al. \cite{FNYSY20}. We show in Theorem \ref{thm:small-size-small-min-cut-correctness} that if $x \in C$ for some min-weight directed cut $(C, V_D \setminus C)$ in $D_G$ with $|C \cap U_V| \leq s$, then running Algorithm \ref{alg:s-sized-small-lambda} on $(D_G,x,k,s)$ will return a min-weight directed cut with constant probability. Thus, running Algorithm \ref{alg:s-sized-small-lambda} on $(D_G,x,k,s)$ for each $x \in U_V$ and returning the best cut found will indeed return a min-weight directed cut in $D_G$ with constant probability; repeating this process $\log n$ times and taking the best cut found will return a min-weight directed cut with high probability. We also show in Theorem \ref{thm:small-size-small-min-cut-correctness} that Algorithm \ref{alg:s-sized-small-lambda} can be implemented to run in time $O(\lambda^3rs^r)$. Thus, running Algorithm \ref{alg:s-sized-small-lambda} $O(\log n)$ times for each $x \in U_V$ and returning the best cut found takes time $\tilde{O}(nk^3rs^r) = \tilde{O}(pk^2rs^r)$. Adding in the time for the base case where $p \leq 512k^2rs^r$, we get a total running time of $\tilde{O}(p\lambda^2rs^r + \lambda^4r^2s^{2r})$.

\begin{algorithm}[ht]
\caption{{SmallSizeSmallMinCut}($D_G,x,k,s$)}\label{alg:s-sized-small-lambda}
\begin{algorithmic}
\State Set all arcs as unmarked
\For{$i$ from $1$ to $k + 1$}
\State $y \gets NIL$
\State Run a new iteration of BFS from $x$ to get a BFS tree $T$ as follows:
\While{the BFS algorithm still has an arc $(u,v)$ to explore}
\If{$(u,v)$ is not marked}
\State Mark $(u,v)$
\If{at least $512k^2rs^r$ arcs are marked}
\State \Return $\bot$
\EndIf
\State With probability $\frac{1}{8r(4s^r+k)}$, stop BFS and set $y \gets v$
\EndIf
\EndWhile
\If{$y = NIL$}
\State \Return $V(T)$
\EndIf
\State Flip the orientation of all arcs on the $x-y$ path in $T$
\EndFor
\State \Return $\bot$
\end{algorithmic}
\end{algorithm}

Theorem \ref{thm:small-size-small-min-cut-correctness} completes the proof of theorem \ref{thm:small-lambda-small-cut}.
%We now show the correctness of Algorithm \ref{alg:s-sized-small-lambda}. %\danupon{You need to assume that $x\in C$ for some of these right? I think it's important to state this clearly.}

\begin{theorem}\label{thm:small-size-small-min-cut-correctness}
Let $(C, V_D \setminus C)$ be a min-weight directed cut in $D_G$ with $|C \cap U_V| \leq s$ and $p\ge 512k^2rs^r$. For $x\in C$, Algorithm \ref{alg:s-sized-small-lambda} returns a min-weight directed cut in $D_G$ with probability at least $\frac{3}{4}$. Moreover, Algorithm \ref{alg:s-sized-small-lambda} can be implemented to run in time $O(\lambda^3rs^r)$. 
\end{theorem}
\begin{proof}
We begin by showing the following claim.
\begin{claim}\label{clm:alg-returns-small-cut}
If Algorithm \ref{alg:s-sized-small-lambda} returns $V(T)$ in iteration $j$ of its for-loop, then $(V(T),V_D \setminus V(T))$ is a directed cut in $D_G$ with weight at most $j-1$. 
\end{claim}
\begin{proof} We note that whenever we flip the arcs in an $x-y$ path, the value of any directed cut $(C, V_D \setminus C)$ with $x \in C$ either decreases by $1$ (if $y \in V_D \setminus C$) or stays the same. We also note that if the algorithm eventually returns $V(T)$, then
the last iteration must have explored all arcs reachable from $x$ without exploring $512k^2rs^r$ arcs. Since $|E_D| \geq p > 512k^2rs^r$, this means that not all arcs of $D_G$ are reachable from $x$, and therefore $(V(T), V_D \setminus V(T))$ is a directed cut in $D_G$. The value of the cut $(V(T), V_D \setminus V(T))$ has decreased by at most $1$ in each previous iteration of BFS run, since this is the only time when the algorithm flips the arcs of a path. Therefore, if $V(T)$ is returned in iteration $j$ of the algorithm's for-loop, the corresponding cut in $D_G$ has weight at most $j-1$.
\end{proof}


By Claim \ref{clm:alg-returns-small-cut}, it suffices to show that with constant probability, Algorithm \ref{alg:s-sized-small-lambda} returns $V(T)$ after $\lambda +1$ iterations of BFS. By Claim \ref{clm:alg-returns-small-cut}, the algorithm cannot return $V(T)$ within $\lambda$ iterations of BFS (since this would imply that there exists a directed cut with weight less than $\lambda$). Therefore, since $\lambda \leq k$, the algorithm will always run at least $\lambda + 1$ iterations of BFS if it does not terminate because of marking $512k^2rs^r$ arcs. %It will not run more than $\lambda+1$ iterations as long as $x \in C$ and every vertex chosen as $y$ is from $V_D \setminus C$.  
If $x \in C$, then whenever the algorithm flips the orientations of all arcs of an $x-y$ path where $y \in V_D \setminus C$, the value of the cut $(C, V_D \setminus C)$ in the resulting graph decreases by $1$. Thus, if $x \in C$ and the algorithm fails to return a min-cut after $\lambda+1$ iterations, either the first $\lambda+1$ iterations marked more than $512k^2rs^r$ arcs, or one of the choices for vertex $y$ chosen within the first $\lambda$ iterations is in $C$.
\begin{claim}\label{clm:failure-prob-too-many-marks}
The probability that Algorithm \ref{alg:s-sized-small-lambda} returns $\bot$ due to marking at least $512k^2rs^r$ arcs within the first $\lambda + 1$ iterations of BFS is at most $1/8$.
\end{claim}
\begin{proof}
The expected number of arcs marked by a single iteration of BFS is $8r(4s^r+k)$, so the expected number of arcs marked by $\lambda+1$ iterations of BFS is \[8(\lambda+1)r(4s^r+k) \leq 8(k+1)r(4s^r+k) \leq 64rk^2s^r.\] Therefore, by Markov's inequality, the probability that at least $512k^2rs^r$ arcs are marked in the first $\lambda+1$ iterations is at most $1/8$.
\end{proof}

\begin{claim}\label{clm:failure-prob-bad-y}
The probability that Algorithm \ref{alg:s-sized-small-lambda} picks a vertex from $C$ as $y$ in some iteration of its execution is at most $1/8$.
\end{claim}

\begin{proof}
If the algorithm never terminates a BFS iteration on an arc with an endpoint in $C$, then it will always choose the vertex $y$ from $V_D \setminus C$. We recall that $|C \cap U_V| \leq s$. Therefore, $|C \cap U_{e_{out}}| \leq 2s^r$, since the number of hyperedges of size at most $r$ over a subset of vertices of size $s$ is at most 
\[
\binom{s}{r} + \binom{s}{r-1} + \binom{s}{r-2} + \dots + \binom{s}{2} \leq s^r + \dots + s^2 \leq 2s^r.
\]
Since $C$ is a min-weight directed cut, we also have that $|C \cap U_{e_{in}}| \leq |C \cap U_{e_{out}}| + \lambda \leq |C \cap U_{e_{out}}| + k$. Also, since $C$ is a min-weight directed cut, we know that for any vertex $v$ in $C \cap U_V$, all of $v$'s neighbors must also be in $C$ (since the arcs between vertices in $U_V$ and $V_D \setminus U_V$ have infinite weight). Thus, every arc which is incident to a vertex in $C$ is incident to a vertex in $C \cap (U_{e_{in}} \cup U_{e_{out}})$. Since each vertex in $U_{e_{in}} \cup U_{e_{out}}$ has degree at most $r$, this means that the total number of arcs which touch vertices in $C$ is at most $r(|C \cap U_{e_{in}}| + |C \cap U_{e_{out}}|) \leq r(4s^r+k)$. Each of these arcs is marked at most once during the execution of the algorithm, and has a $1/(8r(4s^r+k))$ chance of causing BFS to terminate when it is marked. Thus, by union bound, the probability that any of these arcs cause the BFS to terminate (and potentially not flip an arc from the min-cut) is at most $1/8$. \end{proof} 

Combining Claim \ref{clm:failure-prob-too-many-marks} with Claim \ref{clm:failure-prob-bad-y}, 
%we have by a union bound that 
and by union bound, the total probability that the algorithm returns an incorrect answer is at most $1/4$.

%We conclude the proof of Theorem \ref{thm:small-size-small-min-cut-correctness} by analyzing 
Finally, we analyze the runtime of Algorithm \ref{alg:s-sized-small-lambda}. The runtime is dominated by the breadth first searches. There are at most $k+1$ searches, and each breadth first search visits at most $512k^2rs^r$ arcs, so the runtime of 
%a single call to 
Algorithm \ref{alg:s-sized-small-lambda} is $O(\lambda^3rs^r)$. %Thus, running the algorithm $O(\log n)$ times on each $x \in U_V$ and taking the best cut found takes time $\tilde{O}(nk^3rs^r) = \tilde{O}(pk^2rs^r)$. Adding in the time for the base case where $p \leq 512k^2rs^r$, we get a total running time of $\tilde{O}(p\lambda^2rs^r + \lambda^4r^2s^{2r})$.
\end{proof}


%\danupon{It should be helpful to end the section with "proof of Thoerem 4.2"}

%\knote{Wrap up the section. Summarize to say something about the proof of Theorem 4.3. Or clarify the paragraph before Algorithm 4.6 by being explicit about the correctness probability and run-time of Algorithm 4.6.}

\subsubsection{Algorithm for large $\lambda$}
In this section, we prove the following theorem which allows us to find min-cut in hypergraphs where some min-cut has small size. The algorithm is fast if the min-cut value is sufficiently large.

\begin{theorem}\label{thm:big-lambda-small-cut}
Let $s$ be a positive integer, and let $G=(V,E)$ be an $n$-vertex $r$-rank hypergraph of size $p$ with $n \geq 2r$ that has a min-cut $(C,V \setminus C)$ with $|C| \leq s$ and min-cut value $\lambda \geq 900s^r\log n$. Then, there exists a randomized algorithm which takes $G$ and $s$ as input and runs in time $\tilde{O}_r(s^{3r}p)$ to return a min-cut of $G$ with high probability.
\end{theorem}

In the rest of this subsection, let $s$ be a positive integer and let $G=(V, E)$ be an $r$-rank $n$-vertex hypergraph of with $m$ hyperedges and size $p$ that has a min-cut $(C, V\setminus C)$ with $|C|\le s$ and min-cut value $\lambda \geq 900s^r \log n$.
We construct a vertex-weighted bipartite graph $B=(V_B, E_B)$ as follows:
The vertex set of $B$ is given by $V_B := U_V \cup U_E$, and the edge set of $B$ is $E_B$, where $U_V, U_E, E_B$ are defined next.
The vertex set $U_V$ has a vertex $u_v$ for every vertex $v \in V$.
The vertex set $U_E$ has a vertex $u_e$ for every hyperedge $e \in E$.
The edge set $E_B$ has an edge $\{u_v, u_e\}$ for every $v \in V$, $e \in E$ such that the hyperedge $e$ contains the vertex $v$ in $G$. We assign a weight of $\infty$ to each vertex in $U_V$ and a weight of $1$ to each vertex in $U_E$. We note that $|V_B| = m + n$ and $|E_B| = p$. Furthermore, the graph $B$ can be constructed from $G$ in $\tilde{O}(p)$ time.
%We construct a vertex-weighted bipartite graph $B=(U_V\cup U_E, E_B)$ as follows: The vertex set $U_V$ has one vertex $u_v$ for every vertex $v \in V$. The vertices in $U_V$ all have infinite weight. The vertex set $U_E$ has one vertex $u_e$ for every hyperedge $e \in E$. The vertices in $U_E$ all have unit weight. There is an edge $\{u_v, u_e\}\in E_B$ if the hyperedge $e$ contains the vertex $v$ in $G$. 

We call a $3$-partition $(L,S,R)$ of the vertices of $B$ with $|L| \leq |R|$ a {\em vertex separator} if removing $S$ from $B$ disconnects $L$ from $R$. We define the weight of the vertex separator as the weight of $S$. %\danupon{BTW, the definition of separator is a bit tricky when it comes to complete graphs (I was also sloppy in my papers). Maybe it helps to state somewhere that we assume that the graph is not complete because otherwise the problem is trivial?} \cnote{Even if $G$ is complete, $B$ cannot be (since it's bipartite). $U_E$ is always a vertex seperator, so I don't think this is a problem}
Throughout this section, for a vertex $u \in V_B$, we use $N(u)$ to denote $\{v \in U_V \cup U_E \colon \{u,v\} \in E_B \}$ and $N[u]$ to denote $N(u) \cup \{u\}$. 
By the weights that we have assigned to vertices of $B$, we have the following observation:
\begin{observation}\label{obs:subset-of-ue}
Every min-weight separator $(L, S, R)$ in $B$ has $S\subseteq U_E$. 
%Any min-weight vertex separator in $B$ must be a subset of $U_E$.
\end{observation}

The following proposition relates min-cut in $G$ to minimum weight separator in $B$. %\cnote{I'm structuring the propositions here slightly differently from the previous section here. We need the actual mapping between cuts and separators to be defined to state/prove Claim \ref{clm:L-is-small} so we can't just hide the correspondence inside of a proof as we did in Proposition \ref{prop:reduction-to-directed-graph}. }

\begin{proposition}\label{prop:corresponence-between-cuts-and-separators}
The following hold: 
\begin{enumerate}
\item If $(L,S,R)$ is a min-weight separator in $B$, then $(\{v \colon u_v \in L\}, \{v \colon u_v \in R\})$ is a min-cut in $G$. 
\item If $(C, V \setminus C)$ is a min-cut in $G$ with $|C| + |E[C]| \leq |V \setminus C| + |E[V \setminus C]|$, then 
for $L := \{u_v \colon v \in C\} \cup \{u_e \colon e \in E \text{ and } e \subseteq C\}$, $S := \{u_e \colon e \in \delta(C)\}$, and $R := \{u_v \colon v \in V \setminus C\} \cup \{u_e \colon e \in E \text{ and } e \subseteq V \setminus C \}$, the tuple $(L,S,R)$ is a min-weight separator in $B$\knote{; moreover, if $|C|\le s$, then $|L|\le 3s^r$}. 
\end{enumerate}
\end{proposition}

\begin{proof}
Let $(L,S,R)$ be a min-weight separator in $B$. By Observation \ref{obs:subset-of-ue} we have that $S \subseteq U_E$, and therefore $(\{v \colon u_v \in L\}, \{v \colon u_v \in R\})$ is a partition of $V$. Observation \ref{obs:subset-of-ue} also implies that $L \cap U_V$ and $R \cap U_V$ are both nonempty, and therefore $(\{v \colon u_v \in L\}, \{v \colon u_v \in R\})$ is a cut. Every edge $e$ crossing this cut is of the form $e = \{u_x,u_y\}$, where $u_x \in L$ and $u_y \in R$. For such an edge $e$, the vertex $u_e$ is adjacent to vertices in both $L$ and $R$, and therefore, by the definition of a vertex separator, we have that $u_e \in S$. Thus, we have that the weight of the cut $(\{v \colon u_v \in L\}, \{v \colon u_v \in R\})$ is at most $|S|$.

Next, let $(C, V \setminus C)$ be a min-cut in $G$ with $|C| + |E[C]| \leq |V \setminus C| + |E[V \setminus C]|$ \knote{where is this condition used in the rest of the proof?}, and let the sets $L,S,R$ be as defined in the proposition. We note that by the definition of $B$, removing $S$ will disconnect $L$ from $R$, and by assumption $|L| \leq |R|$ \knote{by what assumption?}. Thus, $(L,S,R)$ is indeed a vertex separator. Furthermore, since $S \subseteq U_E$, the weight of $(L,S,R)$ is $|S| = |\delta(C)|$.

The arguments in the previous two paragraphs imply that the min-cut value in $G$ is at most the weight of a min-weight separator in $B$, and the weight of a minimum weight separator in $B$ is at most the min-cut value in $G$ \knote{This is not clear. Why does $G$ have a min-cut satisfying the additional condition?}. Thus, the min-cut value in $G$ is equal to the weight of a min-weight separator in $B$, and so the proposition follows from the arguments in the previous two paragraphs.

\knote{I suggest moving the proof of Claim 4.15 into this proof.} 
\end{proof}

Proposition \ref{prop:corresponence-between-cuts-and-separators} implies the following corollary.

\begin{corollary}\label{cor:reduction-to-bipartite-graph}
An algorithm that runs in time $\tilde{O}(f(p,s,r,\lambda))$ to find a min-weight separator in $B$, for some function $f$, can be used to find a min-cut in $G$ in time $\tilde{O}(p + f(p,s,r,\lambda))$.
\end{corollary}
\begin{proof}
As noted above, $B$ can be constructed from $G$ in $\tilde{O}(p)$ time. Furthermore, by Proposition \ref{prop:corresponence-between-cuts-and-separators}, given a min-weight separator $(L,S,R)$ in $B$ we can construct a min-cut in $G$ in $\tilde{O}(p)$ time.
\end{proof}

The following claim translates our assumption that the min-cut $(C, V \setminus C)$ in $G$ has $|C| \leq s$ into a constraint on a minimum-separator in $B$.

\begin{claim}\label{clm:L-is-small}
If $G$ has min-cut $(C, V \setminus C)$ with $|C| \leq s$, then the corresponding vertex separator $(L,S,R)$ defined in Proposition \ref{prop:corresponence-between-cuts-and-separators} has $|L| \leq 3s^r$. 
\end{claim}

\begin{proof}
The corresponding vertex separator in $B$ has $L = \{u_v \colon v \in C\} \cup \{u_e \colon e \in E \text{ and } e \subseteq C\}$. We have that $|\{u_v \colon v \in C\}| \leq s$, and \[|\{u_e \colon e \in E \text{ and } e \subseteq C\}| \leq \binom{s}{r} + \binom{s}{r-1} \dots \binom{s}{2} \leq s^r + \dots s^2 \leq 2s^r.\]
Thus, $|L| \leq s + 2s^r \leq 3s^r$.
\end{proof}

%\begin{proposition}\label{prop:corresponence-between-cuts-and-separators}
%Let $(C, V \setminus C)$ be a cut in $G$ with $|C| + |E[C]| \leq |V \setminus C| + |E[V \setminus C]|$, let $L := \{u_v \colon v \in C\} \cup \{u_e \colon e \in E \text{ and } e \subseteq C\}$, $S:= \{u_e \colon e \in \delta(C)\}$, and $R := \{u_v \colon v \in V \setminus C\} \cup \{u_e \colon e \in E \text{ and } e \subseteq V \setminus C \}$. Then $(L,S,R)$ is a vertex separator in $B$ with weight $|\delta(C)|$. Furthermore, $(L,S,R)$ is a min-weight separator in $B$ if and only if $(C, V \setminus C)$ is a min-cut in $G$.
%\end{proposition}

%\begin{proof}
%By the definition of $B$, removing $S$ will disconnect $L$ from $R$, and by assumption $|L| \leq |R|$. Thus, $(L,S,R)$ is a vertex separator. Furthermore, since $S \subseteq U_E$, the weight of $(L,S,R)$ is $|S| = |\delta(C)|$.

%If $(C, V \setminus C)$ is a min-cut, then $(L,S,R)$ is a vertex separator with weight $\lambda$, and therefore the minimum weight of a vertex separator in $B$ is at most the min-cut value in $G$. On the other hand if $(L,S,R)$ is a min-weight vertex separator, then $(C, V \setminus C)$ is a cut with the same weight as a min-weight vertex separator, and thus the min-cut value in $G$ is at most the minimum weight of a vertex separator in $G$. Thus, we conclude that the weight of a minimum weight vertex separator in $B$ is the same as the min-cut value in $G$, and therefore $(L,S,R)$ is a min-weight separator in $B$ if and only if $(C, V \setminus C)$ is a min-cut in $G$.
%\end{proof}


%\begin{proposition}\label{prop:reduction-to-bipartite-graph}
%An algorithm that runs in time $\tilde{O}(f(p,s,r,\lambda))$ to find a min-weight separator in $B$, for some function $f$, can be used to find a min-cut in $G$ in time $\tilde{O}(p + f(p,s,r,\lambda))$.
%\end{proposition}
%\begin{proof}
%We first note that every cut $(C, V \setminus C)$ in $G$ with $|C| \leq |V \setminus C|$ has a corresponding vertex separator in $B$, namely $(L, S, R)$, where $L := \{u_v \colon v \in C\} \cup \{u_e \colon e \in E \text{ and } e \subseteq C\}$, $S:= \{u_e \colon e \in \delta(C)\}$, and $R := \{u_v \colon v \in V \setminus C\} \cup \{u_e \colon e \in E \text{ and } e \subseteq V \setminus C \}$. The weight of $(L,S,R)$ is just the weight of $S$, and since $S \subseteq U_E$, this is $|S| = |\delta(C)|$. Therefore, the minimum weight of a vertex separator in $B$ is at most the min-cut value in $G$.

%Next, let $(L,S,R)$ be a min-weight vertex separator in $B$. Let $C := \{v \colon u_v \in L\}$. As shown above, there exists a vertex separator with finite weight. Therefore $S$ cannot include any vertices of weight $\infty$, so $S \subseteq U_E$. Therefore, $V \setminus C = \{v \colon u_v \in R\}$. Since $S$ has minimum weight, we must have that $e \cap C \neq \emptyset$ and $e \cap V \setminus C \neq \emptyset$ for every $u_e \in S$ (otherwise $u_e$ could be moved to $R$ and $(L,S,R)$ would still be a vertex separator). Since $(L,S,R)$ is a vertex separator, $u_e$ must be in $S$ for every $e \in \delta(C)$. Thus, $S = \{u_e \colon e \in \delta(C)\}$, and so, $(C, V \setminus C)$ is a cut of weight $|S|$. Therefore, the min-cut value in $G$ is at most the weight of a min-weight vertex separator in $B$.

%The above arguments imply that the minimum weight of a vertex separator in $B$ is equal to the min-cut value in $G$ and moreover, given a min-weight vertex separator in $B$, we can recover a min-cut in $G$ immediately. The run-time guarantees follow. 
%\end{proof}
%We also have that every set $S \subseteq U_E$ corresponds to a set $F \subseteq E$, and vice-versa \knote{saying `corresponds' without giving the mapping is informal. Avoid this. Phrase similar to the previous section.}. Hence, we have the following observation as well:

%\begin{observation}\label{obs:correspondence-with-bipartite}
%A min-weight separator of $B$ corresponds to a min-cut in $G$. Hence, every algorithm that can find min-weight separator in $B$ can also find a min-cut in $G$.
%\end{observation}

%\knote{Set up what is going to happen in the rest of the section: By Observation ..., in order to prove Theorem ..., it suffices to design an algorithm to find a ... - see paragraph above Algorithm \ref{alg:s-sized-small-lambda}.} 

By Corollary \ref{cor:reduction-to-bipartite-graph} and Claim \ref{clm:L-is-small}, in order to prove Theorem \ref{thm:big-lambda-small-cut}, it suffices to design an algorithm  that runs in time $\tilde{O}_r(s^{3r}p)$ to find a min-weight separator $(L,S,R)$ in the bipartite graph $B$,under the assumption that $|L| \leq 3s^r$. To achieve this, we use a slightly modified version of on algorithm of Li et al. \cite{LNPSY21} to obtain a minor of $B$, which we call a \textit{kernel}, which has the following two properties with high probability:
\begin{enumerate}
    \item A min-weight separator in the kernel can be used to find a min-weight separator in $B$ in $\tilde{O}(p)$ time.
    \item The kernel has at most $9rs^r$ vertices from $U_V$.
\end{enumerate}
The first property means that we can reduce \knote{helps in reducing} the problem of finding a min-weight separator in $B$ to the problem of finding a kernel and of finding a min-weight separator in the kernel. The second property allows us to design an algorithm which finds a min-weight separator in a kernel in time $\tilde{O}(\lambda r^2s^{3r})$.
In Algorithm \ref{alg:find-kernel}, we give a randomized procedure that takes $B$, a set $X \subseteq V$ such that $X \cap L \neq \emptyset$, and an integer $\ell$ with $|L|/2 \leq \ell \leq |L|$ as inputs and returns a kernel. Running this algorithm $O(\log n)$ times with $X = U_V$ for each $\ell \in \{1, 2, 4, \dots, 3s^r \}$ will return a kernel. We show the correctness of Algorithm \ref{alg:find-kernel} in Lemma \ref{lem:alg-finds-kernel}. Unfortunately, the runtime of Algorithm \ref{alg:find-kernel} is $\tilde{O}(|E_H| \cdot |X|)$, which is too slow for our purposes. In Lemma \ref{lem:efficient-kernel}, we show that there is a faster algorithm that returns the same kernel as Algorithm \ref{alg:find-kernel}. Finally, in Lemma \ref{lem:alg-for-min-separator} we
obtain an $\tilde{O}(s^{3r}p)$ time algorithm for finding a min-weight separator in $B$ by combining the algorithm for finding a kernel with an algorithm due to Dinitz \cite{Dinitz06} which finds a min-weight separator in a kernel.

%Our algorithm to achieve this is inspired by an algorithm of Forster et al. \cite{FNYSY20}. We will show that if $x \in C$ for some min-weight directed cut $(C, V_D \setminus C)$ in $D_G$, then running Algorithm \ref{alg:s-sized-small-lambda} on $(D_G,x,k)$ will return a min-weight directed cut with constant probability. Thus, running Algorithm \ref{alg:s-sized-small-lambda} on $(D_G,x,k)$ for each $x \in U_V$ and returning the best cut found will indeed return a min-weight directed cut in $D_G$ with constant probability; repeating this process $\log n$ times and taking the best cut found will return the min-weight directed cut with high probability.

%For a cut $(C, V \setminus C)$, the corresponding vertex separator $(L, S, R)$ in $B$ is given by $L:=\{u_v: v\in C\}\cup \{u_e: e\in E \text{ and } e\subseteq C\}$, $S:= \{u_e: e\in E\text{ and } e\cap C\neq \emptyset, e\cap (V\setminus C)\neq \emptyset\}$ and $R:=\{u_v: v\in V\setminus C\}\cup \{u_e: e\in E \text{ and } e\subseteq V\setminus C\}$.  


We will need the following definitions:

\begin{definition} [\cite{LNPSY21}]A vertex separator $(L,S,R)$ is called an $(X,Y)$-separator if $X \subseteq L, Y \subseteq R$. A minimum weight $(X,Y)$-separator will be denoted as a min $(X,Y)$-separator. A vertex separator $(L,S,R)$ is called a $t$-scratch if it has separator size $|S| \leq t$, $|L| \leq t/(100 \log n)$, and $|S_{low}| \geq 300|L|\log n$, where $S_{low} := \{v \in S : \deg(v) \leq 8t\}$
\end{definition}

\begin{definition}\label{def:kernel}
%\iffalse
Let $H=(V,E)$ be a graph with $n$ vertices and $m$ edges and $x \in V$. %\knote{$T\subseteq V\setminus \{x\}$?}. 
We say that $(H_x,Z_x)$ is a kernel for $H$ if the following hold:
\begin{enumerate}
    \item $H_x$ is a subgraph of the graph obtained from $H$ by contracting some subset $T_x \subseteq V\setminus \{x\}$ into a single vertex $t_x$ such that $H_x$ contains $x$ and $t_x$.
    %\knote{How is $T_x$ related to $T$? I am confused here.}\cnote{T isn't a variable here. I have removed it form the notation for clarity.}
    %\knote{I think you can omit $T$ from the subscript. $H_x$ is a subgraph of $H/T$ for some $T\subseteq V\setminus \{x\}$ such that $H_x$ contains $x$ and the contracted vertex, denoted $t_x$.}
    %\knote{$H_{x, T}$ is a subgraph of $H/T$ such that $H_{x, T}$ contains $x$ and the contracted vertex; we will denote the contracted vertex as $t_x$.} 
    \item $Z_{x}$ is a subset of $V$ such that $(L,S,R)$ is a min $(\{x\},\{t_x\})$-separator in $H_{x}$ iff $(L',S \cup Z_{x},R')$ is a min $(\{x\},T_x)$-separator in $H$, where $L'$ is the component of $V_B \setminus (S \cup Z_{x})$ containing $x$, and $R' := V_B \setminus (L' \cup S \cup Z_x)$. %\knote{min $(\{x\},T)$-separator in $H$? Again, I am confused regarding how $T_x$ is related to $T$.}.
\end{enumerate}
%\fi
%Let $H$ be a graph with $n$ vertices and $m$ edges. Let $x$ be a vertex of $H$, and let $T_x$ be a subset of $V(H) \setminus \{x\}$. Let $H'$ be $H$ with the vertices of $T_x$ contracted into a single vertex $t_x$. Let $H_{x,T}$ be a subgraph of $H'$, and let $Z_{x}$ be a subset of the vertices of $H$, such that a set $Y$ is a min $(\{x\},\{t_x\})$-separator in $H_{x,T}$ iff $Y \cup Z_{x}$ is a min $(\{x\},T_x)$-separator in $H$. We call $(H_{x,T}, Z_{x})$ a kernel. \danupon{I found this definiton hard to read. Perhaps move the last sentence to the front?}
%\knote{The definition of a kernel seems to be a mess. I am not able to follow the rest of this section because of this.}
\end{definition}

Our technique to find a min-weight separator in $B$ is to 
%pick a random $T$ and 
find, for each $x \in U_V$, a kernel with $O(\lambda r s^{2r})$ edges. Algorithm \ref{alg:find-kernel} is a slightly modified version of an algorithm of Li et al. \cite{LNPSY21} for computing the kernel. The difference is that while our algorithm contracts $T_x \cup (N(T_x) \cap U_V)$, their algorithm merely contracts $T_x$.
%\knote{$T_x$ vs $T$? Confusing}. 
We need this additional contraction in order to prove Claim \ref{clm:kernel-is-small}, which bounds the size of the kernel. This bound on the size of the kernel that we obtain is necessary to prove Claim \ref{clm:min-separator-in-kernel}, which shows that we can find a min-weight separator in a kernel efficiently.
Additionally, while Li et al. analyzed the algorithm only for an unweighted graph, we run it on the graph $B$, which has vertex weights (of a special kind). 

\begin{algorithm}[ht]
\caption{{FindKernel}($B,X,\ell$)}\label{alg:find-kernel}
\begin{algorithmic}
\State $T \gets \emptyset$
\For{$v$ in $V(B)$}
\State Add $v$ to the set $T$ with probability $1/(8\ell)$
\EndFor
\For{$x \in X$}
\State $T_x \gets T  \setminus N[x]$
\State Obtain $B'$ from $B$ by contracting the vertices of $T_x \cup (N(T_x) \cap U_V)$ into a single vertex $t_x$
\State $Z_{x} \gets \{v \in V(B') \colon \{x,v\},\{v,t_x\} \in E(B')\}$
\State Obtain $B''$ from $B'$ by deleting the vertices of $Z_{x}$ and the edges that are fully contained in $N(t_x)$ 
\State Obtain $B'''$ from $B''$ by deleting all vertices which are disconnected from $x$ in $B'' \setminus N[t_x]$
\State Obtain $B_{x}$ from $B'''$ by deleting from $B'''$ all neighbors of $t_x$ with degree one 
\EndFor
\State \Return $\{ (B_{x},Z_{x}) \colon x \in X\}$
\end{algorithmic}
\end{algorithm}

We show the following lemma which will be useful to analyze the correctness of the algorithm.
\begin{lemma}\label{lem:Tx-subset-R}
Let $(L,S,R)$ be a min-weight separator in $B$. Let $x \in L$, and let $\ell$ be a positive integer with $|L|/2 \leq \ell \leq |L|$. Let $T$ be a subset of $V(B)$ chosen by sampling each vertex with probability $1/(8\ell)$, and let $T_x = T \setminus N[x]$. Then, we have that $\emptyset \neq T_x \subsetneq R$ with probability $\Omega(1)$.
\end{lemma}
\begin{proof}
By the hypothesis of Theorem \ref{thm:big-lambda-small-cut}, we have that $|S| = \lambda \geq 900s^r\log n$. By Claim \ref{clm:L-is-small}, we have that $|L| \leq 3s^r \leq |S|/2$. We also note that a random vertex separator consisting of the neighbors of a single vertex of $U_V$ has expected size at most $r|U_E|/|U_V|$, so $|S| \leq (r/n)|U_E| \leq |U_E|/2$. Consequently, we have that 
\[|(U_V \cup U_E) \setminus N[x]| \geq |U_E| - |S| - |L|  \geq |U_E| - (|U_E|/2) - (|U_E|/4) \geq |U_E|/4 \geq |S|/4 \geq s^r.\] Since each vertex of $V(B) \setminus N[x]$ is included in $T_x$ with probability $1/(8\ell) \geq 1/24s^r$, it follows that at least one of them will be included in $T_x$ with at least constant probability.

Now we note that since $N(x)$ is a vertex separator in $B$, $|N(x)| \geq \lambda$. Thus, $|(L \cup S) \setminus N[x]| \leq (|L| + \lambda) - \lambda = |L|$. Since each of these vertices is included in $T_x$ with probability at most $1/(8(|L|/2)) = 1/(4|L|)$, the probability that none of them are included is at least a constant.

Since $|R| \geq 1$ by the definition of a vertex separator, and since each vertex of $R$ is included in $T_x$ with probability $1/(8\ell) \leq 1/8$, the probability that at least one vertex of $R$ is excluded from $T_x$ is also at least a constant. 
\end{proof}

Now we show the correctness of Algorithm \ref{alg:find-kernel}.

\begin{lemma}\label{lem:alg-finds-kernel}
Consider executing Algorithm \ref{alg:find-kernel} on input $(B, X, \ell)$ for some positive integer $\ell$ such that $|L|/2 \le \ell \le |L|$, where $X$ is a subset of $U_V$ and $(L, S, R)$ is a min-weight separator in $B$. For $x\in X\cap L$, if the set $T_x$ chosen by the algorithm satisfies $\emptyset \neq T_x \subsetneq R$, then the tuple $(B_x, Z_x)$ returned by the algorithm is a kernel.

%Let $(L,S,R)$ be a min-weight separator in $B$. Let $x \in L$ and $\ell$ be a positive integer with $|L|/2 \leq \ell \leq |L|$. Let $X$ be a subset of $U_V$ containing $x$. 
%If the set $T_x$ chosen by Algorithm \ref{alg:find-kernel} satisfies $\emptyset \neq T_x \subsetneq R$, then running Algorithm \ref{alg:find-kernel} on $(B,X,\ell)$ returns a collection that contains a kernel $(B_{x}, Z_{x})$.
\end{lemma}
\begin{proof}
Suppose that $\emptyset \neq T_x \subsetneq R$. Then, $(L,S,R)$ is a min $(\{x\},T_x)$-separator, and contracting $T_x$ cannot destroy $(L,S,R)$ (or any other min $(\{x\},T_x)$-separator). Let $R'$ be $R$ with the vertices of $T_x \cup (N(T_x) \cap U_V)$ contracted into the single vertex $t_x$. By Observation \ref{obs:subset-of-ue} we have that $S \subseteq U_E$, which means that since $T_x \subseteq R$ then $N(T_x) \cap U_V \subseteq R$ as well. Thus, $(L,S,R')$ is a min-weight separator in $B'$.  %Thus, with constant probability, the weight of a min $(\{x\},t_x)$-separator in $B'$ is the same as the weight of $S$.

By Observation \ref{obs:subset-of-ue}, we have that the weight of the separator $(L,S,R)$ is $|S|$. Consequently, we have the following observation:

\begin{observation}\label{obs:disjoint-paths}
There exist $|S|$ disjoint $x-t_x$ paths in $B'$, each of which visits exactly one vertex from $N(x)$ and exactly one vertex from $N(t_x)$.
\end{observation}

Since every edge in $B'[N(x)]$ or $B'[N(t_x)]$ is not present in any of these paths, removing all of these edges does not affect the weight of a min $(\{x\},\{t_x\})$-separator in $B'$. On the other hand, every vertex $v \in N(x) \cap N(t_x)$ must be included in every $(\{x\},\{t_x\})$-separator in $B'$. Therefore, $(B'',Z_{x})$ is a kernel for $B$. 

By Observation \ref{obs:disjoint-paths}, removing from $B''$ vertices which are disconnected from $x$ in $B'' \setminus N[t_x]$ cannot affect the size of a min $(\{x\},\{t_x\})$-separator, since such vertices cannot participate in any $s-t_x$ paths which use only a single vertex of $N(t_x)$. Thus, $(B''',Z_{x})$ is also a kernel.

Finally, we note that degree one neighbors of $t_x$ cannot participate in any $x-t_x$ paths using only one vertex from $B'''[N[t_x]]$. Thus, again by Observation \ref{obs:disjoint-paths}, removing such vertices does not affect the weight of a min $(\{x\},\{t_x\})$-separator, and thus $(B_{x},Z_{x})$ is a kernel.
\end{proof}

Combining Lemma \ref{lem:Tx-subset-R} with Lemma \ref{lem:alg-finds-kernel} we have that for an appropriate choice of $\ell$, Algorithm \ref{alg:find-kernel} will return a kernel $(B_x, Z_x)$ for each $x \in L$ with at least constant probability. As noted above, we can find an appropriate $\ell$ by running the algorithm for each $\ell \in \{1, 2, 4, \dots, 3s^r \}$, and we can improve the success probability be repeating  this process $O(\log n)$ times.
We next show that the kernel computed by Algorithm \ref{alg:find-kernel} is not too large.

\begin{claim}\label{clm:kernel-is-small}
Let $x\in U_V$ and $\ell \le 3s^r$. If the pair $(B_{x},Z_{x})$ in the collection returned by Algorithm \ref{alg:find-kernel} is a kernel, then $B_{x}$ contains at most $9rs^r$ vertices from $U_V$ with high probability.
\end{claim}

\begin{proof}
Let $(C,V \setminus C)$ be a min-cut in $G$ with $|C| \leq s$. Let $(L,S,R)$ be the corresponding min-weight separator in $B_{x}$ (such a vertex separator exists since $B_{x}$ is a kernel). We know that $|L \cap U_V| \leq s \leq rs^r$ and that $S \subseteq U_E$, so it suffices to show that $|R \cap U_V| \leq 8rs^r$. 

Consider an arbitrary vertex $v \in R \cap U_V$. Since $v$ was not contracted into $t_x$, it must be the case that $v$ was not in $T_x$, and none of $v$'s neighbors were in $T_x$. If $v$ had more than $8\ell \log n$ neighbors in $V(B) \setminus N(x)$, then with high probability, one of the neighbors of $v$ would be in $T_x$. Therefore, with high probability, $v$ has at most $8\ell \log n$ neighbors in $V(B) \setminus N(x)$. We know, however, that $v$ must have at least $\lambda$ neighbors in $B$. Therefore, $v$ must have at least $\lambda - 8\ell \log n$ neighbors in $N(x)$.

Since $x \in L$, we have that $|N(x)| \leq |L| + \lambda \leq 3s^r + \lambda$. Since $x \in U_V$, we also have that $N(x) \subseteq U_E$. Since $G$ has rank $r$, it follows that each vertex in $N(x)$ has degree at most $r$. Thus, the vertices of $N(x)$ collectively have at most $r(3s^r +\lambda)$ edges incident to them. Since each vertex of $R \cap U_V$ is incident to at least $\lambda - 8\ell \log n$ of those edges, we have that 
\[|R \cap U_V| \leq \frac{r(3s^r+\lambda)}{\lambda - 8\ell \log n}.\]

From the hypothesis of Theorem \ref{thm:big-lambda-small-cut}, we have that $\lambda \geq 900s^r \log n$. From the hypothesis of the claim we are proving, we have that $\ell \leq 3s^r$. Therefore, $\lambda - 8\ell \log n \geq \lambda /2$, so

\[
\frac{r(3s^r+\lambda)}{\lambda - 8\ell \log n} \leq \frac{2r(3s^r+\lambda)}{\lambda} \leq 2r(3s^r+1) \leq 8rs^r.\qedhere
\]
\end{proof}

%Next we show that the kernel generated by Algorithm \ref{alg:find-kernel} can be obtained efficiently.
The following lemma will be useful in showing that the kernel generated by Algorithm \ref{alg:find-kernel} can be obtained efficiently.
\begin{lemma}\label{lem:efficient-kernel}
There is a randomized algorithm that takes as input the bipartite graph $B$, a subset $X\subseteq U_V$, and positive integers $\ell, t$, 
chooses a set $T$ according to the same distribution as Algorithm \ref{alg:find-kernel} \knote{chooses a subset $T$ of $V(B)$ by sampling each vertex with probability $1/(8\ell)$}, 
%, and a set $T\subseteq V(B)$ 
and runs in time $\tilde{O}(|E(H)| + |X|t\ell)$ to return a pair $(B_x, Z_x)$ for every $x\in X$. Additionally, the returned collection satisfies the following with high probability: 
\begin{itemize}
    \item For $x\in X$, if $B$ contains a $t$-scratch $(L,S,R)$ with $x \in L$, $|L|/2 \leq \ell \leq |L|$, and $\emptyset \neq T \setminus N[x] \subseteq R$, then the pair $(B_{x},Z_{x})$ returned by the algorithm is a kernel with $|E(B_{x})| = O(t\ell \log p)$ \knote{and $B_x$ contains at most ...}. Moreover, $B_x$ contains at most $9rs^r$ vertices from $U_V$.
\end{itemize}
%\knote{What is $H$? How is it related to $B$?} Let $H$ be a graph, $X \subseteq V(H)$, and $\ell, t \in \mathbb{Z}_+$. There is an algorithm which chooses a set $T$ as in Algorithm \ref{alg:find-kernel} and takes $\tilde{O}(|E(H)| + |X|t\ell)$ time to return a pair $(B_{x},Z_{x})$ for each $x \in X$. For each $x \in X$, if $H$ contains a $t$-scratch $(L,S,R)$ with $x \in L$, $|L|/2 \leq \ell \leq |L|$, and $\emptyset \neq T \setminus N[x] \subseteq R$, then the pair $(B_{x},Z_{x})$ returned by the algorithm is a kernel with $|E(B_{x})| = O(t\ell \log n)$. 

%\knote{Why not simply say: There exists an implementation of Algorithm 4.18 that runs in time ... Moreover, the collection returned by the implementation also guarantees that for each $x\in X$, if $B$ contains a $t$-scratch ..., then the pair ... in the collection is a kernel with $|E(B_x)|=O(t\ell \log n)$.}

%\knote{Also wondering if $|E(B_x)|=O(t\ell \log n)$, where $n$ is the number of vertices in $G$?}
\end{lemma}
\begin{proof}
This follows directly from the results of \cite{LNPSY21}. They design an algorithm (Algorithm 1 in \cite{LNPSY21}) which chooses a set $T$ according to the same distribution as Algorithm \ref{alg:find-kernel}, but uses linear sketching and BFS-like computations starting from $x$ to compute a pair $(B_{x},Z_{x})$ more efficiently than Algorithm \ref{alg:find-kernel}; moreover, if $B$ contains a $t$-scratch $(L,S,R)$ with $x \in L, |L|/2 \leq \ell \leq |L|$, and $\emptyset\neq T \setminus N[x] \subseteq R$, then with high probability the pair $(B_x,Z_x)$ returned by their algorithm is a kernel with $|E(B_{x})| = O(t\ell \log p)$, and this kernel is the pair that would be output by their version of Algorithm \ref{alg:find-kernel} when run on the same input with the same source of randomness.
%if the set $T$ chosen by their algorithm is chosen according to the same distribution as that in Algorithm ..., and for $x\in X$, if $B$ contains ..., then their faster algorithm returns the same kernel as their version of Algorithm ... 

%Furthermore, when using the same random set $T$, their faster algorithm returns the same kernel as their version of Algorithm \ref{alg:find-kernel}. \cnote{specify that we will apply their modification to our algorithm and run that. Then explain why the two differences don't matter.} 

We obtain an algorithm with the guarantees given in the statement of the lemma by applying the modifications described in \cite{LNPSY21} to our version of Algorithm \ref{alg:find-kernel}. There are only two differences between Algorithm \ref{alg:find-kernel} and the corresponding algorithm in \cite{LNPSY21}. First, their algorithm is only for unweighted graphs, while we run Algorithm \ref{alg:find-kernel} on the weighted graph $B$. Second, we contract $T_x' := T_x \cup (N(T_x) \cap U_V)$ rather than just $T_x$. We now show that neither of those differences affects the correctness or runtime of the modified algorithm.

We note that since Algorithm \ref{alg:find-kernel} does not even look at the weights on the vertices, the fact that $B$ is weighted does not affect the runtime of our algorithm. 

The additional contraction of $N(T_x) \cap U_V$ into $t_x$can be performed without increasing the runtime of the algorithm, and as shown in Lemma \ref{lem:alg-finds-kernel} the resulting algorithm still finds a kernel whenever $\emptyset \neq T_x \subsetneq R$. Furthermore, by Claim \ref{clm:kernel-is-small}, this kernel contains at most $9rs^r$ vertices from $U_V$ with high probability. We skip the detailed description and analysis of the faster algorithm for finding kernels, since it is identical to \cite{LNPSY21}.
\end{proof}

The following lemma completes the proof of Theorem \ref{thm:big-lambda-small-cut}.
\begin{lemma}\label{lem:alg-for-min-separator}
There exists a randomized algorithm that runs in time $\tilde{O}(s^{3r}p)$ to find a min-weight separator in $B$ with high probability.
\end{lemma}

\begin{proof}
Let $k$ be the approximation of $\lambda$ obtained by running the algorithm from Theorem \ref{thm:CX-approximation}. To find a min-weight separator in $B$, we run the algorithm from Lemma \ref{lem:efficient-kernel} on $B$ with $t = k+r+300s^r\log n$, and $X = U_V$ for $\Theta(\log n)$ times for each $\ell \in \{ 1,2, 4,8, \dots, 3s^r\}$. Then, for each pair $(B_{x}, Z_{x})$ returned, if $B_{x}$ contains at most $9rs^r$ vertices from $U_V$ then we compute a min $(\{x\}, \{t_x\})$-separator in $B_{x}$. For each such separator $(L,S,R)$, we compute a corresponding separator $(L', S', R')$ in $B$ by setting $S' := S \cup Z_x$, $L'$ to be the component of $V_B \setminus S'$ which contains $x$, and $R' := V_B \setminus (L' \cup S')$. By Definition \ref{def:kernel}, if $(B_x, Z_x)$ is a kernel then $(L',S',R')$ is a min-weight $(\{x\},T_x)$-separator in $B$.
%as well as the corresponding separator in $B$ \knote{How do we find the corresponding separator in $B$? Definition 4.18 is not informative for this.}. 
We return the cheapest \knote{among all computed separators} of all the separators computed.

We first analyze the correctness of our procedure. We will need the following claim:

\begin{claim}\label{clm:min-cut-is-scratch}
Let $(L,S,R)$ be a min-weight separator in $B$ with $|L| \leq 3s^r$. Then $(L,S,R)$ is a $t$-scratch.
\end{claim}

\begin{proof}
Since each min-weight separator in $B$ corresponds to a min-cut in $G$, we know that $|S| = \lambda \leq k \leq t$. By assumption and by our choice of $t$, we have that $|L| \leq 3s^r \leq t/(100\log n)$. By Observation \ref{obs:subset-of-ue}, we must have that $S \subseteq U_E$. Also, by the definition of $B$, every vertex in $U_E$ has degree at most $r$, which is less than $8t$. Therefore, we have that $S_{low} = S$. Thus, $|S_{low}| = |S| = \lambda \geq 900s^r\log n \geq 300|L| \log n$, so $(L,S,R)$ is a $t$-scratch.\end{proof}


Let $(C,V \setminus C)$ be a min-cut in $G$ with $|C| \leq s$. Let $(L,S,R)$ be the corresponding min-weight separator in $B$ (such a vertex separator exists by Proposition \ref{prop:corresponence-between-cuts-and-separators}) \knote{be the min-weight separator in $B$, where the sets $L, S, R$ are as defined in Proposition \ref{prop:corresponence-between-cuts-and-separators}}. By Claim \ref{clm:min-cut-is-scratch}, $(L,S,R)$ is a $t$-scratch. Since we run the algorithm of Lemma \ref{lem:efficient-kernel} $\Theta(\log n)$ times %each for every $x \in U_V$ \knote{we only run it for $X=U_V$. What do you mean by `for every $x\in U_V$'?}, and 
for each $\ell = 1,2,4,8, \dots, 3s^r$, we will run the algorithm $\Theta(\log n)$ times for an 
%$x \in L$ \knote{again, we do not run the algorithm for each vertex $x$} and an 
$\ell \in [|L|/2, |L|]$. By Lemma \ref{lem:Tx-subset-R}, for each $x \in L$, each time we run the algorithm the set $T$ that is chosen satisfies $\emptyset \neq T_x \subsetneq R$ with constant probability, so with high probability this occurs for some $x \in L$ at least once. Lemma \ref{lem:efficient-kernel} tells us that when the algorithm chooses such a $T$, then with high probability it will return a kernel $(B_x, Z_x)$ where $B_x$ has at most $9rs^r$ vertices from $U_V$. %Thus, with high probability, the algorithm finds a kernel. By Claim \ref{clm:kernel-is-small}, this kernel has at most $9rs^r$ vertices from $U_V$ with high probability. 
By Definition \ref{def:kernel}, a min $(\{x\},\{t_x\})$-separator in this kernel corresponds \knote{`corresponds' is unclear} \cnote{I edited the kernel definition to make the correspondence more explicit} to a min $(\{x\},T_x)$-separator in $B$ \knote{a min $(\{x\},\{t_x\})$-separator $(L, S, R)$ in this kernel gives a min $(\{x\}, T_x)$-separator $(L', S\cup Z_x, R')$ in $B$, where $L'$ is the component of $V_B\setminus (S\cup Z_x)$ containing $x$, and $R'=V_B\setminus (L'\cup S\cup Z_x)$}. Since $T_x \subseteq R$, a min $(\{x\},T_x)$-separator in $B$ is in fact a min-weight separator in $B$. Thus, the algorithm finds a min-weight separator in $B$ with high probability.

We now analyze the runtime of our procedure. The algorithm from Lemma \ref{lem:efficient-kernel} runs in time $\tilde{O}(|E_B| + |U_V|(k+r+300s^r)(3s^r)) = \tilde{O}(p + n(\lambda+r+s^r)s^r) = \tilde{O}(p+ps^r +rns^{2r}) = \tilde{O}(ps^r+rns^{2r})$. Running the algorithm $\Theta(\log n)$ times each for $\log(3s^r)$ different values of $\ell$ increases the running time by a factor of $O(\log(3s^r)\log n) = O(r(\log s)(\log n)) = O(r\log^2 n)$ giving us a total runtime of $\tilde{O}(prs^r + r^2ns^{2r})$ to compute all of the kernels. To bound the time to compute a min $(\{x\},\{t_x\})$-separator in each kernel we use the following claim.
\begin{claim}\label{clm:min-separator-in-kernel}
If $(B_{x},Z_{x})$ is a pair returned by the algorithm from Lemma \ref{lem:efficient-kernel} with at most $9rs^r$ vertices from $U_V$ and $O(\lambda r s^{2r})$ edges, then a min $(\{x\},\{t_x\})$-separator in $B_{x}$ can be computed in time $\tilde{O}(\lambda r^2s^{3r})$.%\danupon{Just to be sure: Any kernel returned by the algorithm and Lemma 4.21 will be ok?}
\end{claim}

\begin{proof}
Since $B$ is bipartite, every path of length $d$ in $B$ must visit at least $\lceil d /2 \rceil$ vertices in $U_V$. The graph $B_{x}$ is obtained from a bipartite graph by contracting some subset of vertices. Therefore, except for the vertex $t_x$ created by the contraction, every vertex in $B_{x}$ which is not in $U_V$ must have all of its neighbors in $U_V$. This means that for every path in $d$, every pair of consecutive vertex in the path not including the vertex generated by the contraction must have at least one vertex from $U_V$. Therefore, every path of length $d$ in $B_{x}$ must visit at least $\lceil (d-2)/2 \rceil$ vertices from $U_V$. By the assumption of the claim, $B_{x}$ contains $O(rs^r)$ vertices from $U_V$. Thus, every path in $B_{x}$ has length $O(rs^r)$. 

Therefore, we can use Dinitz's algorithm to efficiently find a min $(\{x\},\{t_x\})$-separator in $B_{x}$ \cite{Dinitz06}. Since the lengths of paths in $B_{x}$ are bounded by $O(rs^r)$, the number of blocking flows found by Dinitz's algorithm is also $O(rs^r)$. Each blocking flow can be found in time proportional to the number of edges in $B_{x}$, and by 
%Lemma \ref{lem:efficient-kernel} this is $O(t\ell \log p) = \tilde{O}(\lambda rs^{2r})$. 
assumption this is $\tilde{O}(\lambda rs^{2r})$.
Therefore, the total runtime of Dinitz's algorithm on a $B_x$ is $\tilde{O}(\lambda r^2s^{3r})$. 
\end{proof}

Let $(B_x, Z_x)$ be a kernel for $B$ returned by the algorithm from Lemma \ref{lem:efficient-kernel}. By Claim \ref{clm:kernel-is-small} we have that $B_x$ contains at most $9rs^r$ vertices from $U_V$ with high probability, and by Lemma \ref{lem:efficient-kernel} we have that $B_x$ has $O(\lambda r s^{sr})$ edges with high probability. By Claim \ref{clm:min-separator-in-kernel} we can compute a min-weight separator for a single $B_x$ with at most $9rs^r$ vertices from $U_V$ and $O(\lambda r s^{sr})$ in time $\tilde{O}(\lambda r^2s^{3r})$. Thus, we can compute a min-weight separator for each $B_x$ with at most $9rs^r$ vertices from $U_V$ and $O(\lambda r s^{sr})$ edges in time $\tilde{O}_r(s^{3r}\lambda n) = \tilde{O}_r(s^{3r}p)$, and with high probability this will compute a min-weight separator in a kernel.

\end{proof}

\subsection{Expander Decomposition Based Min-Cut}\label{sec:large-min-cut}
In this section, we give an algorithm to find connectivity in hypergraphs in which every min-cut has large size. In order to analyze the run-time of our algorithm, we need to bound the run-time to implement trim and shave operations. This is summarized in the following claim.

\begin{claim}\label{clm:efficient-trim-and-shave}
Let $G=(V,E)$ be an $n$-vertex $r$-rank hypergraph of size $p$ with $p \geq n$, and let $\mathcal{X}=\{X_1, \dots, X_k\}$ be a collection of disjoint subsets of $V$. Then there exists a deterministic algorithm which takes as input an  $G$  and $\mathcal{X}$, and runs in time $O(pr)$ to return $\{\trim(X_1), \dots, \trim(X_k)\}$ and $\{\shave(X_1), \dots, \shave(X_k)\}$.
\end{claim}
\begin{proof}


For $v\in V$, let $part(v):=i$ if $v\in X_i$ and $0$ otherwise. For $e\in E$, let $epart(e):=i$ if $e\subseteq X_i$ and $0$ otherwise. Let $d_{\mathcal{X}}(v):=d_{X_i}(v)$ if $v\in X_i$ and $0$ otherwise and $\delta_{\mathcal{X}}(v):=\delta_{X_i}(v)$ if $v\in X_i$ and $\emptyset$ otherwise. We also recall that the degree of a vertex in $G$ is denoted by $d(v)$. The functions $part:V\rightarrow \{0, \dots, k\}$, $d: V \rightarrow \mathbb{Z}_+$, $d_{\mathcal{X}} : V \rightarrow \mathbb{Z}_{\geq 0}$, and $\delta_{\mathcal{X}}: V \rightarrow 2^E$ can be found in $O(p)$ time using Algorithm \ref{alg:trim-shave-helper}. 

\begin{algorithm}\label{alg:trim-shave-helper}
\caption{TrimShaveHelper$(G=(V,E),\mathcal{X}=\{X_1, \dots, X_k\})$}
\begin{algorithmic}
\ForAll{$v \in V$}
\State $part(v), d(v), d_{\mathcal{X}}(v) \gets 0$
\State $\delta_{\mathcal{X}}(v) \gets \emptyset$
\EndFor
\For{$i=1,\ldots, k$}
\ForAll{$v \in X_i$}
\State $part(v) \gets i$
\EndFor
\EndFor
\ForAll{$e \in E$}
\State $v \gets$ an arbitrary vertex of $e$
\State $epart(e) \gets part(v)$
\ForAll{$u \in e \setminus \{v\}$}
\If{$part(u) \neq part(v)$}
\State $epart(e) \gets 0$
\EndIf
\EndFor
\If{$epart(e) \neq 0$}
\ForAll{$v \in e$}
\State $d_{\mathcal{X}}(v) \gets d_{\mathcal{X}}(v) + 1$
\State Add $e$ to $\delta_{\mathcal{X}}(v)$
\EndFor
\EndIf
\EndFor
\State \Return $part,d,d_X,\delta_X$
\end{algorithmic}
\end{algorithm}

We claim that Algorithm \ref{alg:trim-shave-helper} can be implemented to run in time $O(p)$. We note that looping over all of the vertices takes time $O(n)$. Since the sets $X_i$s are disjoint, looping over all the vertices of each $X_i$ also takes time $O(n)$. Looping over all edges and within each edge looping over all vertices in the edge takes time $O(\sum_{e \in E} |e|) = O(p)$. Since $n \leq p$, the complete algorithm can be implemented to run in time $O(p)$.

We use Algorithm \ref{alg:shave} to perform the $\shave$ operation. Since the sets $X_i$s are disjoint, iterating over all vertices of each $X_i$ takes time $O(n)$, so the portion of the algorithm outside of the call to \textsc{TrimShaveHelper} can be implemented to run in time $O(p)$, and therefore the whole algorithm can be as well.

\begin{algorithm}
\caption{ShaveAlgorithm$(G=(V,E), \mathcal{X}=\{X_1, \dots, X_k\}$}\label{alg:shave}
\begin{algorithmic}
\State $part,d,d_{\mathcal{X}},\delta_{\mathcal{X}} \gets \textsc{TrimShaveHelper}(G,\mathcal{X})$
\For{$i=1, \dots, k$}
\ForAll{$v \in X_i$}
\If{$d_{\mathcal{X}}(v) \leq (1-1/r^2)d(v)$}
\State Remove $v$ from $X_i$
\EndIf
\EndFor
\EndFor
\State \Return $\mathcal{X}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{TrimAlgorithm$(G=(V,E), \mathcal{X}=\{X_1, \dots, X_k\})$} \label{alg:trim}
\begin{algorithmic}
\State $x,y,d,d_{\mathcal{X}},\delta_{\mathcal{X}} \gets \textsc{TrimShaveHelper}(G,\mathcal{X})$
\State $T \gets \emptyset$
\State $F \gets V$
\While{$T \cup F \neq \emptyset$}
\If{$T \neq \emptyset$}
\State Let $v \in T$ be arbitrary
\State Remove $v$ from $T$ and from $X_{part(v)}$
\State $part(v) \gets 0$
\ForAll{$e \in \delta_{\mathcal{X}}(v)$}
\For{$u \in e \setminus \{v\}$}
\State Remove $e$ from $\delta_{\mathcal{X}}(u)$
\State $d_{\mathcal{X}}(u) \gets d_{\mathcal{X}}(u) - 1$
\If{$d_{\mathcal{X}}(u) < d(u)/2r$ and $u \not\in T$}
\State Add $u$ to $T$
\EndIf
\EndFor
\EndFor
\Else
\State Let $v \in F$ be arbitrary
\State remove $v$ from $F$
\If{$d_{\mathcal{X}}(v) < d(v)/2r$ and $part(v) \neq 0$}
\State Add $v$ to $T$
\EndIf
\EndIf
\EndWhile
\State \Return $\mathcal{X}$
\end{algorithmic}
\end{algorithm}
We use Algorithm \ref{alg:trim} to perform the $\trim$ operation. Here the set $F$ stores vertices that the algorithm has yet to examine, and $T$ stores vertices that the algorithm has determined must be trimmed. The values of $d_{\mathcal{X}}(v)$ and $\delta_{\mathcal{X}}(v)$ are updated as vertices are trimmed, and whenever $d_{\mathcal{X}}(v)$ changes for a vertex $v$, the algorithm verifies whether that vertex $v$ should be trimmed. Removing vertices from $X_i$ cannot increase $d_{X_i}(v)$ for any vertex $v \in X_i$. Therefore, if a vertex $v$ satisfies $d_{X_i}(v) < d(v) / 2r$ when $v$ is added to $T$, $v$ will still satisfy this inequality when it is actually removed from $X_i$.
We note that each vertex is chosen at most once as the arbitrary vertex from $F$, since whenever a vertex is chosen from $F$ it is removed from $F$ and never added back to it. Whenever a vertex $v$ is chosen from $T$, it is removed from $T$, and $part(v)$ is set to $0$. Since the algorithm only adds a vertex $v$ to $T$ only if $part(v) \neq 0$, each vertex is chosen at most once as the arbitrary vertex from $T$.

The case of choosing a vertex from $F$ can be implemented to run in constant time since we perform an arithmetic comparison and a constant number of set additions and removals. 
When the algorithm selects a vertex from $T$, it iterates over all hyperedges of that vertex which are currently in $X_{part(v)}$. For each of these hyperedges $e$, all iterations of the innermost \textbf{for} loop can be implemented to run in time $O(|e|)$. Thus, the total time spent processing a vertex $v$ from $T$ is $O(\sum_{e \in \delta(v)} |e|)$. Since each vertex is processed in $T$ at most once, the total time to process all of the vertices is $O(\sum_{v \in V}\sum_{e\in \delta(v)}|e|)=O(pr)$.
\end{proof}

%Let $G=(V,E)$ be an $r$-rank hypergraph of size $p$ that has a min-cut $(C,V \setminus C)$ with $|C| \leq s$. Then, there exists a randomized algorithm $\textsc{SmallSizeMinCut}$ which takes as input $G$ and $s$ and runs in time $\tilde{O}_r(s^{6r}p)$ to return a min-cut of $G$ with high probability.

\begin{theorem}\label{thm:large-mincut-algo}
Let $G=(V,E)$ be an $n$-vertex $r$-rank hypergraph of size $p$ with min-cut value $\lambda$ such that $n > r2^{r+1}$ and $\lambda > 6r^2(4r^2)^r$
and every min-cut $(C,V \setminus C)$ in $G$ has $\min\{|C|,|V \setminus C|\} > r-\log \lambda / \log n$. Then there exists a randomized algorithm which takes $G$ as input
%There exists a randomized algorithm that takes as 
%input a positive integer $k$ and an $r$-rank $n$-vertex hypergraph $G=(V,E)$ with $p := \sum_{e \in E} |e|$ and connectivity $\lambda$ 
and runs in time 
\[
\tilde{O}_r\left(p + (\lambda n)^{1+o(1)} + \min\left\{\frac{n^{r+r \cdot o(1)}}{\lambda^{\frac{r}{r-1}}}, \lambda^{\frac{r-3}{r-1}+o(1)}n^{2+o(1)}, \lambda^{\frac{5r-7}{4r-4}+o(1)}n^{\frac{7}{4}+o(1)}\right\}\right),
\]
to return a min-cut of $G$ with high probability.
%to return a cut of $G$. If %$\lambda >n> r(4r^2)^r$ 
%$n > r2^{r+1}$ and $\lambda > 6r^2(4r^2)^r$
%and every min-cut $(C,V \setminus C)$ has $\min\{|C|,|V \setminus C|\} > r-\log \lambda / \log n$, then the returned cut is a min-cut with high probability. 

\end{theorem}

\begin{proof}
We will use algorithms from Theorems \ref{thm:CX-approximation}, \ref{thm:CX-sparsifier}, \ref{thm:FPZ-min-cut}, and \ref{thm:CQ-min-cut} and Lemma \ref{lem:efficient-expander-decomp} to find a min-cut. We use \textsc{CXApproximation} to find a constant-approximation $k$ for the min-cut value. Next, we use \textsc{CXSparsifier}$(G,k)$ to get a graph $G'$ with size $p_1=O(kn)=O(\lambda n)$. Next, we find an expander decomposition $\cX$ of $G'$ with respect to the parameter $\phi:=(6r^2/\delta)^{1/(r-1)}$. We then apply the trim operation on $\cX$ followed by $3r^2$ shave operations to obtain a collection $\cX''$ of disjoint subsets of $V$. We contract all these subsets and run either \textsc{FPZMinCut}, \textsc{CXMinCut}, or \textsc{CQMincut} on the resulting hypergraph to find a min-cut. We present the pseudocode of our approach in Algorithm \ref{alg:exp-decomp-min-cut}.

\begin{algorithm}
\caption{ExpDecompMinCut$(G)$}\label{alg:exp-decomp-min-cut}
\begin{algorithmic}
\State $k \gets \textsc{CXApproximation}(G)$
\State $G' \gets \textsc{CXSparsifier}(G,k)$
\State $\delta' \gets \min_{v \in V} d_{G'}(v)$
\State $\phi \gets \min\{(6r^2/\delta')^{1/(r-1)}, 1/(r-1)\}$
\State $\mathcal{X} \gets$ \textsc{ExpanderDecomposition}$(G',\phi)$
\State $\mathcal{X'} \gets \textsc{TrimAlgorithm}(G',\mathcal{X})$
\State $\mathcal{X}'' \gets \textsc{ShaveAlgorithm}(\mathcal{X}')$
\For{$i=2, \ldots, 3r^2$}
\State $\mathcal{X}'' \gets \textsc{ShaveAlgorithm}(\mathcal{X''})$
\EndFor
\State Let $G''$ be the hypergraph obtained by contracting each set $X''_i \in \mathcal{X''}$ into a single vertex
\If{$k^{\frac{2r-3}{r-1}} \geq n^{r-2}$ and $k^{\frac{9}{4}+\frac{1}{2r-2}} \geq n^{r-\frac{1}{2}}$}
\State \Return $\text{FPZMinCut}(G'')$
\Else
\If{$k^{\frac{1}{4}+\frac{3}{2r-2}} \geq n^{\frac{3}{2}}$ or $k=0$}
\State \Return $\text{CXMinCut}(G'')$
\Else
\State \Return $\text{CQMinCut}(G'')$
\EndIf
\EndIf
\end{algorithmic}
\end{algorithm}

We now prove the correctness of Algorithm \ref{alg:exp-decomp-min-cut}. 
By Theorem \ref{thm:CX-approximation} we have that $k > \lambda$. Therefore, by Theorem \ref{thm:CX-sparsifier}, the min-cut value in $G'$ is $\lambda$, and the min-cuts in $G'$ are exactly the min-cuts of $G$. Consequently, the min-degree $\delta'$ in $G'$ is at least the connectivity $\lambda$. Let $(C, V \setminus C)$ be an arbitrary min-cut in $G'$. By Lemma \ref{lem:efficient-expander-decomp}, for every $i \in [k]$, we have that 
\begin{align*}
\delta' \geq \lambda &\geq \left|E^o_{G'}(X_i \cap C, X_i \cap (V \setminus C))\right| \\
&\geq \min\left\{\left(\frac{6r^2}{\delta'}\right)^{\frac{1}{r-1}},\frac{1}{r-1}\right\} \min \{\vol_{G'}(X_i \cap C), \vol_{G'}(X_i \setminus C)\} \\
&\geq \min\left\{\left(\frac{6r^2}{\delta'}\right)^{\frac{1}{r-1}},\frac{1}{r-1}\right\}  \delta' \min \{|X_i \cap C|, |X_i \setminus C|\}.
\end{align*}
Thus, $\min\{|X_i \cap C|, |X_i \setminus C| \} \leq \max\{(\delta'/6r^2)^{1/(r-1)},r-1\}$.
Therefore, by Claim \ref{clm:trim-bound}, and $3r^2$ repeated applications of Claim \ref{clm:shave-bound}, we have that $\min\{|X''_i \cap C|, |X''_i \cap (V \setminus C)|\} = 0$. In particular, this means that contracting each $X''_i$ does not destroy $(C, V \setminus C)$, so $\delta(C)$ is still a min-cut set in $G''$. Since contraction cannot decrease the capacity of any cut, this implies that every min-cut in $G''$ is a min-cut in $G'$, and thus Algorithm \ref{alg:exp-decomp-min-cut} returns a correct answer.

We now bound the run-time of Algorithm \ref{alg:exp-decomp-min-cut}. 
By Theorem \ref{thm:CX-approximation}, \textsc{CXApproximation} runs in time $O(p)$ to return $k\le 3\lambda$. By Theorem \ref{thm:CX-sparsifier},  \textsc{CXSparsifier} also runs in time $O(p)$ to return a hypergraph 
$G'=(V, E')$ of size $p_1:= \sum_{e \in E'} |e|=O(kn)=O(\lambda n)$ and having min-degree $\delta'\ge \lambda$. By Lemma \ref{lem:efficient-expander-decomp}, we obtain an expander decomposition $\cX$ of $G'$ in time 
\[
O\left(p_1^{1+o(1)}\right)
\]
such that the number of hyperedges of $G'$ intersecting multiple parts of $\cX$ is 
$
O(r\phi p_1^{1+o(1)})
$. 
By Claim \ref{clm:efficient-trim-and-shave}, we can implement a $\trim$ operation followed by $3r^2$ $\shave$ operations to obtain a collection $\cX''$ of disjoint subsets of $V$ in time $O(p_1r \cdot 3r^2) = O(p_1r^3)$.   
By Claim \ref{clm:hyperedges-lost-to-trim} and $3r^2$ repeated applications of Claim \ref{clm:hyperedges-lost-to-shave} (similar to the proof of Theorem \ref{thm:number-of-hyperedges-in-mincuts}), we have that 
$
|E''| = O(4r^{9r^2+1}\phi p_1^{1+o(1)})
$.
Since contraction cannot decrease the degree of any vertex, every vertex in $G''=(V'',E'')$ has degree at least $\delta'$. Therefore, the number of vertices $n_2$ in $G''$ must satisfy $n_2\delta' \le \sum_{v\in V''}d_{G''}(v)=\sum_{e\in E''}|e|\le r|E''|$, which implies that 
\[
n_2
= O\left( \frac{4r^{9r^2+2}\phi p_1^{1+o(1)}}{\delta'}\right)
= O\left( \frac{4r^{9r^2+2}\phi p_1^{1+o(1)}}{\lambda}\right).
\]
Let $p_2 := \sum_{e \in E''} |e|$. Since contraction cannot increase the size of the hypergraph, we have that $p_2 \leq p_1$. Moreover, contraction does not increase the rank and hence the rank of $G''$ is at most $r$. Therefore, the run-time of \textsc{FPZMinCut} on $G''$ is 
\begin{align*}
    \tilde{O}\left(p_2  + n_2^r\right)
    &= \tilde{O}\left(p_1 + \left( \frac{4r^{9r^2+2}\phi p_1^{1+o(1)}}{\lambda}\right)^r  \right) \\
    &= \tilde{O}\left( \lambda n + \frac{r^{11r^3}(\lambda n)^{r(1+o(1)}\phi^r}{\lambda^r} \right) \\
    &= \tilde{O}\left(\lambda n + r^{11r^3}\lambda^{r \cdot o(1)}n^{r(1+ o(1))}\phi^r \right) \\
    &= \tilde{O}\left(\lambda n + \frac{r^{15r^3}n^{r(1+o(1))}}{\lambda^{\frac{r}{r-1}-r \cdot o(1)}} \right).
\end{align*}
The second equation is by the bound on $p_1$, and the last equation is by the setting of $\phi$ and using the fact that $\delta'\ge \lambda$. 

The run-time of $\textsc{CXMinCut}$ on $G''$ is  
\begin{align*}
O(\lambda n_2^2) &= O\left( \frac{16r^{18r^2+4}\phi^2 p_1^{2+o(1)}}{\lambda}\right) \\
&= O \left( \frac{r^{19r^2}(\lambda n)^{2+o(1)}\phi^2}{\lambda} \right) \\
&= O\left(r^{19r^2}\lambda^{1+o(1)}n^{2+o(1)}\phi^2 \right) \\
&= O\left( r^{20r^2}\lambda^{\frac{r-3}{r-1}+o(1)}n^{2+o(1)}  \right).
\end{align*}
Again, the second equation is by the bound on $p_1$, and the last equation is by the setting of $\phi$ and the fact that $\delta' \geq \lambda$.

Let $m_2$ be the number of edges in $G''$. If $G''$ is connected, we have that $n_2 \leq p_2$, and therefore $(m_2 + n_2) \leq 2p_2$. Since $p_2 \leq rm_2$, this bound is tight, up to a factor of $r$.
%We note that, assuming $G''$ is connected, we have $m_2 + n_2 \leq 2p_2$. 
Since we run \textsc{CQMinCut} on $G''$ only if $k \neq 0$ (and thus $G''$ is connected), the run-time of $\textsc{CQMinCut}$ on $G''$ is
\begin{align*}
    \tilde{O}\left(\sqrt{p_1n_2(m_2+n_2)^{1.5}}\right) &= \tilde{O}\left(\sqrt{p_1n_2(2p_2)^{1.5}}\right) \\
    &= \tilde{O}\left(\sqrt{p_1^{2.5}n_2 } \right) \\
    &= \tilde{O}\left(p_1^{1.25}n_2^{0.5} \right) \\
    &= \tilde{O}\left((\lambda n)^{1.25}\left(\frac{4r^{9r^2+2}\phi (\lambda n)^{1+o(1)}}{\lambda}\right)^{0.5} \right) \\
    &=\tilde{O}\left(r^{4.5r^2+1}\lambda^{1.25+o(1)}n^{1.75+o(1)}\left(\frac{6r^2}{\lambda}\right)^{\frac{1}{2(r-1)}} \right) \\
    &=\tilde{O}\left(r^{4.5r^2+2}\lambda^{\frac{5r-7}{4r-4}+o(1)}n^{1.75+o(1)} \right).
\end{align*}
The fourth equation is by the bound on $p_1$, and the second-to-last equation is by the setting of $\phi$ and the fact that $\delta' > \lambda$.

Since the algorithm runs whichever of $\textsc{FPZMinCut}$, $\textsc{CXMinCut}$, and $\textsc{CQMinCut}$ is faster, the overall runtime is
\begin{align*}
    &\tilde{O}\left(p+p_1^{1+o(1)} + r^3p_1 + \min \left\{ \lambda n + \frac{r^{15r^3}n^{r(1+o(1))}}{\lambda^{\frac{r}{r-1}-r \cdot o(1)}}, r^{20r^2}\lambda^{\frac{r-3}{r-1}+o(1)}n^{2+o(1)}, r^{4.5r^2+2}\lambda^{\frac{5r-7}{4r-4}+o(1)}n^{\frac{7}{4}+o(1)}  \right\}\right) \\
    = &\tilde{O}\left(p + (\lambda n)^{1+o(1)} + r^3\lambda n + \min \left\{ \frac{r^{15r^3}n^{r(1+o(1))}}{\lambda^{\frac{r}{r-1}-r \cdot o(1)}}, r^{20r^2}\lambda^{\frac{r-3}{r-1}+o(1)}n^{2+o(1)}, r^{4.5r^2+2}\lambda^{\frac{5r-7}{4r-4}+o(1)}n^{\frac{7}{4}+o(1)}  \right\} \right)
\end{align*}

The run-time bound stated in the lemma follows by observing that $\lambda n \le \delta n \le p$, where $\delta$ is the min-degree of the input graph. 
\end{proof}

\begin{remark}\label{remark:det-exp-decomp-min-cut}
We can obtain a deterministic counterpart of Theorem \ref{thm:large-mincut-algo} by
modifying the last step of Algorithm \ref{alg:exp-decomp-min-cut} to always call \textsc{CXMinCut} instead of \textsc{PFZMinCut} or \textsc{CQMinCut}.
The resulting algorithm has a run-time of 
\[
\tilde{O}_r \left(p + (\lambda n)^{1 + o(1)} + \lambda^{\frac{r-3}{r-1}+o(1)}n^{2+o(1)}\right).
\]
\end{remark}




\subsection{Proof of Theorem \ref{theorem:algo}}\label{sec:main-algorithm}
In this section we restate and prove Theorem \ref{thm:min-cut-algorithm}. 

\minCutAlgorithm*
\begin{proof}

%If $n\le r(4r^2)^r$, then the result follows immediately using \textsc{SlowMinCut} from Theorem \ref{thm:slow-min-cut}. If $\lambda $
If $n\le r2^{r+1}$, then the result follows immediately using \textsc{SlowMinCut} from Theorem \ref{thm:slow-min-cut}. If $\lambda \leq 6r^2(4r^2)^r$, then the result follows by first sparsifying the hypergraph with the algorithm $\textsc{CXSparsifier}$ from Theorem \ref{thm:CX-sparsifier} and then running Chekuri and Quanrud's algorithm $\textsc{CQMincut}$ from Theorem \ref{thm:CQ-min-cut}. Hence, we may assume that $n > r2^{r+1}$ and $\lambda > 6r^2(4r^2)^r$
%Also, if $\lambda\le n$, then the result follows by using Chekuri and Xu's algorithm \textsc{CXMinCut} stated in Section \ref{sec:prelims} \cnote{This was true when our claimed runtime was $\tilde{O}_r(p + \min\left\{\lambda n^2, n^r/\lambda \right\})$, but it doesn't hold for the improved runtime. Do we actually have a way to handle the case when $\lambda < n$?}. Hence, we may assume that $\lambda >n>r(4r^2)^r$. 

Our algorithm finds an approximation for the min-cut value, then uses the sparsifier from Theorem \ref{thm:CX-sparsifier} to reduce the size of the hypergraph to $O(\lambda n)$. At this point we either run the min-cut algorithm from Theorem \ref{thm:slow-min-cut} or use the two algorithms we have described in the previous two sections, whichever will run faster. We give pseudocode for our approach in Algorithm \ref{alg:main-alg}. This algorithm uses the algorithms from Theorems 
\ref{thm:CX-approximation}, \ref{thm:CX-sparsifier}, \ref{thm:new-small-mincut-algo} and \ref{thm:large-mincut-algo}.

\begin{algorithm}
\caption{MinCut$(G)$}\label{alg:main-alg}
\begin{algorithmic}
\State $k \gets \textsc{CXApproximation}(G)$
\State $G' \gets \textsc{CXSparsifier}(G, k)$
\State $(C_1, V\setminus C_1) \gets$ \textsc{SmallSizeMinCut}$(G',r-(\log(k)-2)/ \log n)$
\State $(C_2, V \setminus C_2) \gets \textsc{ExpDecompMinCut}(G')$
\State $C \gets \arg\min\{|\delta_G(C_1)|, |\delta_G(C_2)|\}$ 
\State \Return $(C, V \setminus C)$
\end{algorithmic}
\end{algorithm}

We first show that Algorithm \ref{alg:main-alg} returns a min-cut. By Theorem \ref{thm:CX-approximation}, we have that $\lambda <k \le 3\lambda$. Therefore, by Theorem \ref{thm:CX-sparsifier}, every min-cut in $G$ has capacity $\lambda$ in $G'$ and every other cut has capacity greater than $\lambda$ in $G'$. Thus, the set of min-cuts in $G'$ is exactly the same as the set of min-cuts in $G$. It remains to show that the cut $(C, V \setminus C)$ returned by the algorithm is a min-cut in $G'$. 
We distinguish two cases: (i) Suppose some min-cut in $G'$ has size at most $r-\log \lambda/ \log n$. We have that $r-\log \lambda/ \log n \leq r- \log (k/3)/\log n \leq r - (\log(k)-2)/\log n$. Therefore, by Theorem \ref{thm:new-small-mincut-algo}, the call to \textsc{SmallMinCut} returns a min-cut in $G'$, and thus $(C, V \setminus C)$ is a min-cut in $G'$. (ii) Suppose that every min-cut in $G'$ has size greater than $r-\log \lambda/ \log n$. Then, by Theorem \ref{thm:large-mincut-algo}, the algorithm $\textsc{ExpDecompMinCut}$ returns a min-cut in $G'$ and thus, $(C, V \setminus C)$ is a min-cut in $G'$. 

We now analyze the runtime of Algorithm \ref{alg:main-alg}. By Theorems \ref{thm:CX-approximation} and \ref{thm:CX-sparsifier}, the computation of $k$ and $G'$ can be done in $O(p)$ time. Also by Theorem \ref{thm:CX-sparsifier}, the algorithm $\textsc{CXSparsifier}$ returns a hypergraph $G'=(V,E')$ with $\vol_{G'}(V) = \sum_{e \in E'} |e| = O(kn)$. 
By Theorem \ref{thm:new-small-mincut-algo}, the runtime of $\textsc{SmallSizeMinCut}(G', r-(\log(k)-2)/\log n)$ is
\[
\tilde{O}_r((r-\frac{\log(k)-2}{\log n})^{6r}kn) = \tilde{O}_r(\lambda n) = \tilde{O}_r(p)
\]
By Theorems \ref{thm:CX-approximation} and \ref{thm:CX-sparsifier}, the min-cut value in $G'$ is still $\lambda$. Therefore, by Theorem \ref{thm:large-mincut-algo}, the runtime of   $\textsc{ExpDecompMinCut}(G')$ is 
\begin{align*}
&\tilde{O}_r\left(p + (\lambda n)^{1+o(1)} + \min\left\{\frac{n^{r+r \cdot o(1)}}{\lambda^{\frac{r}{r-1}}}, \lambda^{\frac{r-3}{r-1}+o(1)}n^{2+o(1)}, \lambda^{\frac{5r-7}{4r-4}+o(1)}n^{\frac{7}{4}+o(1)} \right\}\right) \\ =\, &\hat{O}_r\left(p + \min\left\{\frac{n^r}{\lambda^{\frac{r}{r-1}}}, \lambda^{\frac{r-3}{r-1}}n^2, \lambda^{\frac{5r-7}{4r-4}}n^{\frac{7}{4}} \right\}\right)\end{align*}
Thus, the overall runtime of the algorithm is
\[\hat{O}_r \left(p + \min\left\{\frac{n^r}{\lambda^{\frac{r}{r-1}}},\lambda^{\frac{r-3}{r-1}}n^2, \lambda^{\frac{5r-7}{4r-4}}n^{\frac{7}{4}} \right\}\right)\]
\end{proof}

\begin{remark}
We obtain the deterministic counterpart of Theorem \ref{theorem:algo} by using the deterministic version of \textsc{ExpDecompMinCut} in Algorithm \ref{alg:main-alg} (that was discussed in Remark \ref{remark:det-exp-decomp-min-cut}) and by using the deterministic algorithm for \textsc{SmallMinCut} described in Appendix \ref{sec:det-small-size-min-cut} instead of the algorithm from section \ref{sec:small-size-min-cut}. The resulting algorithm has a run-time of 
\[
\hat{O}_r\left(p + \min\left\{\lambda n^2, \lambda^{\frac{r-3}{r-1}}n^2 + \frac{n^{r}}{\lambda} \right\}\right).
\]
\end{remark}
